DPconv: Super-Polynomially Faster Join Ordering

We revisit the join ordering problem in query optimization. The standard exact algorithm, DPccp, has a worst-case running time of $O(3^n)$. This is prohibitively expensive for large queries, which are not that uncommon anymore. We develop a new algorithmic framework based on subset convolution. DPconv achieves a super-polynomial speedup over DPccp, breaking the $O(3^n)$ time-barrier for the first time. We show that the instantiation of our framework for the $C_\max$ cost function is up to 30x faster than DPccp for large clique queries.

==> algorithms/dp_conv_max.tex <==
\begin{algorithm}
    \DontPrintSemicolon
  \caption{\texttt{DPconv[max]}: Optimal cost w.r.t. $\Cmax$ in $O(2^n n^2 \log  W \tau_{\max})$-time}\label{algo:dp_conv_max}
  \begin{algorithmic}[1]
  \STATE \textbf{Input:} Query graph $Q = (V, E)$
  \STATE \textbf{Output:} Optimal cost value w.r.t. $\Cmax$
  \STATE $\gamma^* \gets 0$
  \STATE $p \gets \log \texttt{DPconv}(Q,\:\textsc{RoundDown}(c))$
  \WHILE{$p \geq 0$}
      \STATE $\gamma^* \gets \gamma + 2^p$
      \FOR{\textbf{each} $S \subseteq V$}
        \STATE \lIf{$c(S) \in [2^p, 2^{p + 1} - 1]$} {$c(S) \gets c(S) - 2^p$}
        \STATE \lElseIf{$c(S) < 2^p$}{$c(S) \gets 0$}
        \STATE \lElse{$c(S) \gets +\infty$}
      \ENDFOR
      \STATE $p \gets \log \texttt{DPconv}(Q, \textsc{RoundDown}(c))$
  \ENDWHILE
  \RETURN\!$\gamma^*$
  \end{algorithmic}
\end{algorithm}

==> algorithms/fast_cmax.tex <==
\begin{algorithm}
    \DontPrintSemicolon
    \caption{Fast implementation of the $\oplus$-operator for $\Cmax$}\label{algo:fast_c_max_semi-ring}
    \begin{algorithmic}[1]
    \STATE \textbf{Input:} TODO
    \STATE \textbf{Output:} TODO

    \STATE ret[0] = $xs[0]_{+} \cdot ys[0]_{+}$
    \STATE sum $\gets$ $ys[0]_{+}$
    \STATE mars $\gets$ $xs[0]_{+}$
    \FOR{ i in 1 $\ldots$ size(xs)}
      \STATE ret[i] $\gets$ ret[i] + sum $\cdot\:xs[i]_{+}$
      \STATE mars $\gets$ mars + $xs[i]_{+}$
      \STATE ret[i] $\gets$ ret[i] + mars $\cdot\:ys[i]_{+}$
      \STATE sum $\gets$ sum + $ys[i]_{+}$
    \ENDFOR
    \RETURN\!$\text{ret}$
  \end{algorithmic}
\end{algorithm}
